Physics at a 100 TeV pp collider: Higgs and EW symmetry breaking studies

This report summarises the physics opportunities for the study of Higgs bosons and the dynamics of electroweak symmetry breaking at the 100 TeV pp collider.

==> 00-Intro/report.tex <==
\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 00-Intro/section-new.tex <==
\section{Foreword}
A 100~TeV $pp$ collider is under consideration, by the high-energy
physics community~\cite{benedikt,cepc_website},
as an important target for the future development
of our field, following the completion of the LHC and High-luminosity
LHC physics programmes. The physics opportunities and
motivations for such an ambitious
project were recently reviewed in~\cite{Arkani-Hamed:2015vfh}. The
general considerations on the strengths and reach of very high energy
hadron colliders have been introduced long ago in the classic pre-SSC
EHLQ review~\cite{Eichten:1984eu}, and a possible framework to establish the
luminosity goals of such accelerator was presented recently
in~\cite{Hinchliffe:2015qma}.

The present document is the result of an extensive study, carried out
as part of the Future Circular Collider (FCC) study towards a Conceptual
Design Report, which includes separate Chapters dedicated to Standard
Model physics~\cite{SMreport}, physics of the Higgs boson and EW symmetry
breaking (this paper), physics beyond the Standard
Model~\cite{Golling:2016gvc}, physics of heavy ion
collisions~\cite{Dainese:2016gch} and physics with the FCC injector
complex~\cite{inj-report}. Studies on the physics programme of an
$e^+e^-$ collider (FCC-ee) and $ep$ collider (FCC-eh)
at the FCC facility are proceeding
in parallel, and preliminary results are documented
in~\cite{Gomez-Ceballos:2013zzn} (for FCC-ee) and
in~\cite{AbelleiraFernandez:2012cc} (for the LHeC precursor of FCC-eh).

\section{Introduction} 
\label{sec:intro}
Despite its impressive success in accounting for a wide range of
experimental observations, the Standard Model (SM) leaves many of our most
important questions unanswered:
\begin{itemize}
\item Why does the universe contain more matter than anti-matter?
\item What is the identity of the dark matter and what are its interactions?
\item Why are the masses of neutrinos so much smaller than those of all other known elementary fermions?
\end{itemize}
The discovery~\cite{Aad:2012tfa,Chatrchyan:2012xdj}
of the Higgs-like scalar~\cite{Englert:1964et,Higgs:1964ia,Higgs:1964pj,Guralnik:1964eu,Higgs:1966ev,Kibble:1967sv} at the LHC highlights
additional theoretical puzzles.  The scalar sector is the ``obscure"
sector of the SM, in the sense that it is the least understood part of
the theory.  The principles dictating its structure are still
unclear. This is to be contrasted with the gauge sector, which
logically follows from an elegant symmetry principle and has all the
features of a fundamental structure. Not surprisingly, many of the
open problems of the SM are connected to the Higgs sector. For
example, the stability of the Higgs mass~\cite{Weisskopf:1939zz} and
of the Electroweak (EW) scale in general against UV-sensitive
radiative corrections motivates additional symmetry structures near
the TeV scale. To address these questions, possible theoretical extensions of
the SM have been proposed. Their experimental manifestations can be
direct, via the 
production of new particles, or indirect, via deviations of the Higgs
properties from their SM predictions.

With its higher energy and the associated increase in parton
luminosity, a 100 TeV pp collider would provide an unprecedented
potential to both detect new particles, and to explore in detail the
Higgs boson properties, uniquely complementing the capabilities at the
LHC and possible future $e^+e^-$ colliders. This Chapter is dedicated
to a first assessment of this potential.

In the first Section we review what is known today about the
production properties of the 125~GeV Higgs boson at 100~TeV. We
present evidence that the increased energy does not introduce
uncertainties larger than those already established from the studies
for the
LHC~\cite{Dittmaier:2011ti,Dittmaier:2012vm,Heinemeyer:2013tqa}.
Furthermore, the large production rates available at 100~TeV open new
opportunities to optimize the balance between statistical
uncertainties, background contamination, and systematic uncertainties
of both theoretical and experimental origin.  The second Section
illustrates these ideas with a few concrete examples of possible
precision attainable at 100~TeV. These are not
intended to provide a robust and definitive assessment of the ultimate
goals; this would be premature, since both the theoretical landscape
(higher-order corrections, resummations, PDFs, and event simulation
tools in general) and the future detectors' performance potential are
far from being known. Rather, theese examples suggest possible new
directions, which on paper and in the case of idealized analysis
scenarios offer exciting opportunities to push the precision and the
reach of Higgs physics into a domain that will hardly be attainable by
the LHC (although some of these ideas might well apply to the HL-LHC
as well).

The third Section addresses the determination of the Higgs self-coupling
and the measurement of the Higgs potential. This is important for
several reasons. In the SM, the shape of the Higgs potential is
completely fixed by the mass and vacuum expectation value of the Higgs
field.  Therefore, an independent measurement of the trilinear and
quadrilinear Higgs self-interactions provides important additional
tests of the validity of the SM.  This test is quite
non-trivial. Indeed, discussed in the final Section, in many
Beyond-the-SM (BSM) scenarios sizable corrections to the Higgs
self-couplings are predicted, which, in some cases, can lead to large
deviations in multi-Higgs production processes but not in other
observables. In these scenarios, an analysis of the non-linear Higgs
couplings can be more sensitive to new-physics effects than other
direct or indirect probes~\cite{Grober:2010yv,Contino:2012xk}.
This Section includes an overview of the production rates for
multiple Higgs production, including those of associated production
and in the vector-boson fusion channel.
This is followed by a detailed up-to-date study of the possible
precision with which the triple Higgs coupling can be measured, and a
first assessment of the potential to extract information on the
quadruple coupling.

Determining the structure of the Higgs potential is also important to
understand the features of the EW phase transition, whose properties
can have significant implications for cosmology. For instance, a
strong first order transition could provide a viable scenario to
realize baryogenesis at the EW scale (see for
example~\cite{Trodden:1998ym} and references therein).  In the SM the
EW transition is known to be rather weak (for a Higgs mass $m_h
\gtrsim 90$~GeV, only a cross-over is predicted), so that it is not
suitable for a successful baryogenesis. Many BSM scenarios, however,
predict modifications in the Higgs potential that lead to first order
EW transitions, whose strength could allow for a viable baryogenesis.
An additional aspect related to the structure of the Higgs potential
is the issue of the stability of the EW vacuum (see for instance
Ref.~\cite{Degrassi:2012ry}). The final Section of this Chapter will
address these questions in great detail.
This Section will also study the impact of studies in the Higgs sector
on the issue of Dark Matter, or the origin of neutrino masses, and on
naturalness. Extensions of the SM affecting the Higgs sector of the
theory often call for the existence of additional scalar degrees of
freedom, either fundamental or emergent.  Such \emph{Beyond the SM
  (BSM) Higgs sectors} frequently involve new singlet or
electroweak-charged fields, making their discovery at the LHC
challenging. The prospects for their direct observation at 100~TeV
will be presented in the final part of the Section.


The results and observations presented throughout this document, in
addition to put in perspective the crucial role of a 100~TeV $pp$
collider in clarifying the nature of the Higgs boson and electroweak
symmetry breaking, can be used as benchmarks to define detector
performance goals, or to exercise new analysis concepts (focused, for
example, on the challenge of tagging multi-TeV objects such as top and
bottom quarks, or Higgs and gauge bosons).  Equally important, they
will hopefully trigger complete analyses, as well as new ideas and
proposals for interesting observables. Higgs physics at 100~TeV will
not just be a larger-statistics version of the LHC, it will have the
potential of being a totally new ballgame.






==> 01-SM/authors.tex <==
\author{
Editors: \\
R.~Contino$^{1,2}$,\, 
D.~Curtin$^{3}$,\,
A.~Katz$^{1,4}$,\,
M.~L.~Mangano$^{1}$,\,
G.~Panico$^{5}$,\,
M.~J.~Ramsey-Musolf$^{6,7}$,\, 
G.~Zanderighi$^{1}$\,
\\
Contributors: \\
C.~Anastasiou$^{8}$,\,
W.~Astill$^{9}$,\,
J.~K.~Behr$^{10,11}$,\,
W.~Bizon$^{9}$,\,
P.~S.~Bhupal~Dev$^{12}$,\,
D.~Bortoletto$^{10}$,\,
Q.-H.~Cao$^{13,14,15}$,\,
F.~Caola$^{1}$,\,
J.~Chakrabortty$^{16}$,\, 
C.-Y.~Chen$^{17,18,19}$,\, 
S.-L.~Chen$^{15,20}$,\, 
F.~Dulat$^{8}$,\,
G.~Bambhaniya$^{21}$,\, 
D.~Buttazzo$^{22}$\,  
D.~de~Florian$^{23}$,\, 
C.~Englert$^{24}$,\,  
J.~A.~Frost$^{10}$,\, 
B.~Fuks$^{25}$,\,  
T.~Gherghetta$^{26}$,\, 
G.~Giudice$^{1}$,\,
J.~Gluza$^{27}$,\,  
N.~Greiner$^{28}$,\,
H.~Gray$^{29}$,\,
N.~P.~Hartland$^{10}$,\,
C.~Issever$^{10}$,\,
T.~Jeli\'nski$^{27}$,\,  
A.~Karlberg$^{9}$,\,
J.~H.~Kim,$^{30,31,32}$,\, 
F.~Kling$^{33}$,\,  
A.~Lazopoulos$^{8}$,\,
S.~J.~Lee$^{34,35}$,\, 
Y.~Liu$^{13}$,\,
G.~Luisoni$^{1}$,\,
J.~Mazzitelli$^{23,36}$,\, 
B.~Mistlberger$^{1}$,\,
P.~Monni$^{9}$,\,
K.~Nikolopoulos$^{37}$,\,  
R.~N~Mohapatra$^{3}$,\,
A.~Papaefstathiou$^{1}$,\,
M.~Perelstein$^{38}$,\,  
F.~Petriello$^{39}$,\,  
T.~Plehn$^{40}$,\,  
P.~Reimitz$^{40}$,\, 
J.~Ren$^{41}$,\, 
J.~Rojo$^{10}$,\,
K.~Sakurai$^{42}$,\, 
T.~Schell$^{40}$,\, 
F.~Sala$^{43}$,\, 
M.~Selvaggi$^{44}$,\, 
H.-S.~Shao$^{1}$,\,
M.~Son$^{30}$,\,
M.~Spannowsky$^{42}$,\,
T. Srivastava$^{16}$,\,
S.-F.~Su$^{33}$,\,
R. Szafron$^{45}$,\, 
T.~Tait$^{46}$,\,   
A.~Tesi$^{47}$,\,   
A.~Thamm$^{48}$,\,  
P.~Torrielli$^{49}$,\,
F.~Tramontano$^{50}$,\,
J.~Winter$^{51}$,\,
A.~Wulzer$^{52}$,\,
Q.-S.~Yan$^{53,54,55}$,\,
W.~M.~Yao$^{56}$,\,
Y.-C.~Zhang$^{57}$,\,
X.~Zhao$^{53}$,\,
Z.~Zhao$^{53,58}$,\,
Y.-M.~Zhong$^{59}$
\vspace*{2cm}
}

\institute{
$^{1}$ CERN, TH Department, CH-1211 Geneva, Switzerland. \\
$^{2}$ EPFL, Lausanne, Switzerland. \\
$^{3}$Maryland Center for Fundamental Physics, Department of Physics, University of Maryland, College
Park, MD 20742, USA\\
$^{4}$Universit\'{e} de Gen\`{e}ve, Department of Theoretical Physics and Center for Astroparticle Physics,
24 quai E. Ansermet, CH-1211, Geneva 4, Switzerland\\
$^{5}$ IFAE, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Barcelona\\
$^{6}$ Amherst Center for Fundamental Interactions, Physics Department,University of Massachusetts Amherst, Amherst, MA 01003, USA\\
$^{7}$ Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, CA 91125 USA\\
$^{8}$ Institute for Theoretical Physics, ETH Z\"urich,  8093 Z\"urich, Switzerland \\
$^{9}$ Rudolf Peierls Centre for Theoretical Physics, 1 Keble Road, University of Oxford, UK \\
$^{10}$ Physics Department, 1 Keble Road, University of Oxford, United Kingdom\\
$^{11}$ Deutsches Elektronen-Synchrotron (DESY), Notkestrasse 85, D-22607 Hamburg, Germany\\
$^{12}$ Max-Planck-Institut f\"ur Kernphysik, Saupfercheckweg 1,
D-69117 Heidelberg, Germany\\
$^{13}$ Department of Physics and State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, China\\
$^{14}$ Collaborative Innovation Center of Quantum Matter, Beijing 100871, China\\
$^{15}$ Center for High Energy Physics, Peking University, Beijing 100871, China}
$^{16}$  Department of Physics, Indian Institute of Technology, Kanpur-208016, India\\
$^{17}$ Department of Physics, Brookhaven National Laboratory, Upton, New York 11973, USA\\
$^{18}$ Department of Physics and Astronomy, University of Victoria, Victoria, British Columbia V8P 5C2, Canada\\
$^{19}$ Perimeter Institute for Theoretical Physics, Waterloo, Ontario N2J 2W9, Canada\\
$^{20}$ Key Laboratory of Quark and Lepton Physics (MoE) and Institute of Particle Physics, Central China Normal University, Wuhan 430079, China\\
$^{21}$ Theoretical Physics Division, Physical Research Laboratory, Ahmedabad-380009, India\\
$^{22}$ Physik-Institut, Universit\"at Z\"urich, CH-8057 Z\"urich, Switzerland \\ 
$^{23}$ International Center for Advanced Studies (ICAS), UNSAM, Campus Miguelete, 25 de Mayo y Francia, (1650) Buenos Aires, Argentina\\
$^{24}$ SUPA, School of Physics and Astronomy, University of Glasgow,
Glasgow G12 8QQ, UK \\
$^{25}$ Sorbonne Universit\'es, UPMC Univ.~Paris 06, UMR 7589, LPTHE, F-75005 Paris, France.  CNRS, UMR 7589, LPTHE, F-75005 Paris, France \\
$^{26}$ School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA\\
$^{27}$ Institute of Physics, University of Silesia, Uniwersytecka 4, 40-007 Katowice, Poland\\
$^{28}$ Physik Institut, Universit\"at Z\"urich, Winterthurerstrasse 190, CH-8057 Z\"urich, Switzerland \\
$^{29}$ CERN, EP Department, CH-1211 Geneva, Switzerland. \\
$^{30}$ Department of Physics, Korea Advanced Institute of Science and Technology, 335 Gwahak-ro, Yuseong-gu, Daejeon 305-701, Korea \\
$^{31}$ Center for Theoretical Physics of the Universe, IBS, 34051 Daejeon, Korea\\
$^{32}$ Center for Axion and Precision Physics Research, IBS, 34141 Daejeon, Korea \\
$^{33}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{34}$ Department of Physics, Korea University, Seoul 136-713, Korea\\
$^{35}$ School of Physics, Korea Institute for Advanced Study, Seoul 130-722, Korea\\
$^{36}$ Departamento de Fisica and IFIBA, FCEyN, Universidad de
Buenos Aires, (1428) Pabellon 1 Ciudad Universitaria, Capital Federal,
Argentina \\
$^{37}$ School of Physics and Astronomy, University of Birmingham,
Birmingham, B15 2TT, United Kingdom \\
$^{38}$Laboratory for Elementary Particle Physics, Cornell University,
Ithaca, NY 14853, USA\\
$^{39}$ 
Northwestern University, Department of Physics and Astronomy, 2145
Sheridan Road, 
Evanston, Illinois 60208-3112, USA\\
$^{40}$ Institut f\"ur Theoretische Physik, Universit\"at Heidelberg, Germany \\
$^{41}$ Department of Physics, University of Toronto, Toronto, Ontario, Canada M5S1A7\\
$^{42}$ IPPP, Department of Physics, University of Durham, Science Laboratories, South Road, Durham, DH1 3LE, UK\\
$^{43}$ 2LPTHE, CNRS, UMR 7589, 4 Place Jussieu, F-75252, Paris, France\\
$^{44}$ Centre for Cosmology, Particle Physics and Phenomenology CP3, Universit\'e Catholique de Louvain, Chemin du Cyclotron, 1348 Louvain la Neuve, Belgium\\
$^{45}$ Department of Physics, University of Alberta, Edmonton, AB
T6G 2E1, Canada\\
$^{46}$ Department of Physics and Astronomy, University of California, Irvine, CA 92697, USA\\
$^{47}$ Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA\\
$^{48}$ PRISMA Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany\\
$^{49}$ Dipartimento di Fisica, Universit\`a di Torino, and INFN, Sezione di Torino, \\
Via P.~Giuria~1, I-10125, Turin, Italy \\
$^{50}$ Universit\`a di Napoli ``Federico II'' and INFN, Sezione di
Napoli, 80126 Napoli, Italy \\
$^{51}$Department of Physics and Astronomy, Michigan State University,
East Lansing, MI 48824, USA\\
$^{52}$Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova and
INFN, Sezione di Padova, via Marzolo 8, I-35131 Padova, Italy\\
$^{53}$ School of Physical Sciences, University of Chinese Academy of Sciences, Beijing 100049, P. R. China\\
$^{54}$ Center for High-Energy Physics, Peking University, Beijing 100871, P. R. China\\
$^{55}$ Center for future high energy physics, Chinese Academy of Sciences 100049, P. R. China\\
$^{56}$ Lawrence Berkeley National Lab (LBNL), One Cyclotron Rd, Berkeley, CA94720, USA\\
$^{57}$ Service de Physique Th\'eorique, Universit\'e Libre de Bruxelles, Boulevard du Triomphe, CP225, 1050 Brussels, Belgium\\
$^{58}$ Department of Physics, University of Siegen, 57068 Siegen, Germany\\
$^{59}$ C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, New York 11794, USA\\
}


==> 01-SM/ggHpt_orig.tex <==
\subsection{Higgs plus jet and Higgs $p_T$ spectrum in $gg\to H$}
%%%%%\footnote{Editor: Caola}}
\label{sec:H_ggHpt}
In this section we study the production of Higgs in gluon fusion in association
with one extra jet and more in general we analyze the transverse momentum spectrum of the Higgs.

%
\subsubsection{Jet veto efficiencies}
At 100 TeV, extra jet radiation is enhanced and a significant fraction of Higgs boson events
is produced in association with one or more extra jets. To quantify this statement, in Fig.~\ref{fig:efficiency}
we plot the jet veto efficiency at 100 TeV, defined as the fraction of exactly 0-jet events in
the total Higgs sample
\begin{equation}
\epsilon(p_{\rm{t,veto}}) \equiv 1-\frac{\Sigma_{\rm 1-jet,incl} (p_{\rm t,veto})}{\sigma_{\rm tot}},
\end{equation}
as well as the one-jet inclusive cross section as a function of the jet transverse momentum requirement,
$\Sigma_{\rm 1-jet,incl} (p_{\rm t,veto}) \equiv \int_{p_{\rm t,veto}}^{\infty}
\frac{{\rm d} \sigma}{{\rm d}p_{\rm t,jet}} {\rm d} p_{\rm t,jet}$. 
%
\begin{figure}[h]
\includegraphics[width=0.45\textwidth]{figs/ggHpt/matched-v-nnlo-efficiency-100TeV.pdf}
\includegraphics[width=0.45\textwidth]{figs/ggHpt/matched-v-nnlo-1jetxs-100TeV.pdf}
\caption{Jet veto efficiency (left) and 1-jet inclusive cross section for Higgs production
in gluon fusion at 100 TeV, see text for details.}\label{fig:efficiency}
\end{figure}
%
Throughout this section, jets are reconstructed with the anti-$k_t$
algorithm with $R=0.4$. No rapidity cut on the jet is applied. The
efficiency and one-jet cross section shown in
Fig. ~\ref{fig:efficiency} are computed both in pure fixed-order
perturbation theory (red/solid) and matched to NNLL
$\ln m_H/p_{\rm t,veto}$ and LL jet-radius $\ln R$ resummation
(blue/hatched). The uncertainties are obtained with the
Jet-Veto-Efficiency method. %, see~\cite{} for details.
%
For a jet $p_t$ of $\sim 60~{\rm GeV}$, Fig.~\ref{fig:efficiency}
shows that about $30\%$ of the total Higgs cross section comes from
events with one or more jets. Also, for jet transverse momenta larger
than $\sim 60$~GeV it is also clear from Fig.~\ref{fig:efficiency}
that pure fixed-order perturbation theory provides an excellent
description of the jet efficiencies and cross sections. All-order
resummation effects become sizable at smaller transverse momenta,
where however soft physics effects like underlying event and MPI may
play an important role at the centre-of-mass energies considered in
this report.
%

\subsubsection{The Higgs $p_T$ spectrum}
We now study the Higgs cross-section as a function of a cut on the transverse momentum of the Higgs
boson $\sigma(p_{T,H}>p_{t,{\rm cut}})$. 
\begin{figure}
\includegraphics[width=0.45\textwidth]{figs/ggHpt/ptH_2TeV_mtopvseft_diff}
\hfil
\includegraphics[width=0.45\textwidth]{figs/ggHpt/ptH_8TeV_mtopvseft_diff}
\\
\includegraphics[width=0.45\textwidth]{figs/ggHpt/ptH_2TeV_mtopvseft}
\hfil
\includegraphics[width=0.45\textwidth]{figs/ggHpt/ptH_8TeV_mtopvseft}
\caption{Higgs differential (top) and integrated (bottom) $p_t$
  spectrum, comparing the results of the calculation with the exact
  $m_{top}$ dependence, and in the effective field theory (EFT) approximation.}\label{fig:sigma_pt}
\end{figure}
In Fig.~\ref{fig:sigma_pt}, we compare the LO distributions for the
effective $m_t\to\infty$ and full (resolved top) theory. In the
following, we use as central scale  
$\mu = {\sqrt{m_H^2+p_{t,H}^2}}/{2}$. With this scale, the impact of
higher order corrections is 
expected to be minimized, as shown for the effective theory in
Fig.~\ref{fig:scale_Hpt}.  
Since Fig.~\ref{fig:sigma_pt} shows that the effect of finite quark
effects is much more important than  
perturbative corrections, for the predictions in this section we will
use the LO prediction with 
full quark mass dependence, which is the best result available right
now. Fig.~\ref{fig:scale_Hpt} 
suggests that this should be a good approximation in the whole $p_t$
range considered here up 
to a factor of about 2.

\begin{figure}
\includegraphics[width=0.5\textwidth]{figs/ggHpt/plot_mudep_lowpt.pdf}
\includegraphics[width=0.5\textwidth]{figs/ggHpt/plot_mudep_highpt.pdf}
\caption{Scale variation study. Note that at high $p_t$ there is a
  large $\mathcal O(1)$ uncertainty 
coming from PDFs.}\label{fig:scale_Hpt}
\end{figure}

From the result in Fig.~\ref{fig:sigma_pt} we can read off the value
of the transverse momentum 
for which the cross-section is larger than $\sim$ 1~fb$^{-1}$ or
$\sim$ 1~ab$^{-1}$.  
The results are documented
in Tab.~\ref{tab:sigmaBR_pt}.

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
& $\sigma(p_t>p_{t,cut})\times BR = 1~{\rm fb}^{-1}$ & $\sigma(p_t>p_{t,cut})\times BR = 1~{\rm ab}^{-1}$ \\
\hline
$H\to b\bar b$ & $p_{t,cut} = 1860~{\rm GeV}$ & $p_{t,cut} = 5380~{\rm GeV}$ \\
$H\to \tau\bar \tau$ & $p_{t,cut} = 1240~{\rm GeV}$ & $p_{t,cut} = 3950~{\rm GeV}$ \\
$H\to \mu^+\mu^-$ & $p_{t,cut} = 340~{\rm GeV}$ & $p_{t,cut} = 1570~{\rm GeV}$ \\
\hline
$H\to c\bar c$ & $p_{t,cut} = 1070~{\rm GeV}$ & $p_{t,cut} = 3520~{\rm GeV}$ \\
$H\to s\bar s$ & $p_{t,cut} = 350~{\rm GeV}$ & $p_{t,cut} = 1600~{\rm GeV}$ \\
\hline
$H\to gg$ & $p_{t,cut} = 1320~{\rm GeV}$ & $p_{t,cut} = 4130~{\rm GeV}$ \\
$H\to \gamma\gamma$ & $p_{t,cut} = 620~{\rm GeV}$ & $p_{t,cut} = 2350~{\rm GeV}$ \\
$H\to Z\gamma$ & $p_{t,cut} = 570~{\rm GeV}$ & $p_{t,cut} = 2200~{\rm GeV}$ \\
$H\to W^+W^-$ & $p_{t,cut} = 1560~{\rm GeV}$ & $p_{t,cut} = 4700~{\rm GeV}$ \\
$H\to ZZ$ & $p_{t,cut} = 1050~{\rm GeV}$ & $p_{t,cut} = 3470~{\rm GeV}$ \\
\hline
\end{tabular}
\caption{Cross-section times branching ratio as a function of $p_{t,cut}$. Each entry
corresponds to the $p_{t,cut}$ value.}\label{tab:sigmaBR_pt}
\end{table}

At 100 TeV, the rapidity spectrum is much wider than at 13 TeV, as
shown in Fig.~\ref{fig:yHyj}.
for both the Higgs and the leading jet distributions.
 
\begin{figure}
\includegraphics[width=0.49\textwidth]{figs/ggHpt/plot_yh.pdf}
\includegraphics[width=0.49\textwidth]{figs/ggHpt/plot_y1.pdf}
\caption{Higgs and leading jet rapidity distributions, normalized to the total
cross section.}
\label{fig:yHyj}
\end{figure}

%Other results to be added
%\begin{itemize}
%\item channel comparison
%\item differential distributions for $H\to WW$
%\item off-shell 
%\end{itemize}


==> 01-SM/prospects_summary.tex <==
\subsection{Final remarks}
The primary goal of the
  studies shown in this Section was to show that, while theoretical systematics in
  hadronic collisions are typically the key limitation to Higgs
  precision physics, there are examples where these can be reduced
  even using today's knowledge, and there are examples where the large
  statistics allows to identify robust observables (e.g. ratios of
  BRs) where the precision can in principle achieve the percent level.
    What must be explored is the extent to which the performance of
    future detectors can match this accuracy.
    The results shown here can then serve as benchmarks for the definition of
  the performance goals of future detectors.

  To first
  approximation, we believe that the basic experimental systematics
  that appear in the extraction of absolute cross sections
  (luminosity, tagging and identification efficiencies for the various
  physics objects, backgrounds) will cancel in the measurement of
  several Higgs production ratios. the
  ${N_H}/{N_Z}$ ratio. Given the cuts we introduced, the $t$,
  $\bar{t}$ and $H/Z$ objects will be separated from each other, and
  have $p_T$ and angular distributions very similar in the $t\bar{t}H$
  and $t\bar{t}Z$ cases. Therefore the leading uncertainties in the
  $b$ or top tagging efficiencies, or in other important quantities
  such as lepton isolation and identification, will cancel. The
  remaining systematics will arise  from the differences
  in detector response due to the slight kinematical differences. We
  find it reasonable to expect that, for a quantity such as the $b$
  tagging efficiency, which is typically known to within few percent,
  it should be possible to control the relative difference between the
  efficiency in $H\to b\bar{b}$ and in $Z\to b\bar{b}$ decays. No
  study at the level of what can be done using the simplified tools
  available to us can give compelling proof of this statement, and we
  propose that studies of systematics for these ratios of efficiencies
  should be interesting goals for more realistic performance studies of
  future detectors.

We would also like to add that the huge rates at 100~TeV will give
  many high-statistics control samples, which can be used for
  data-driven precise determinations of backgrounds or
  efficiencies. As a relevant example, we briefly mention here the
  case of: 
%
\begin{equation}
 pp \to Z Z \to \ell^+ \ell^- b \bar{b} \; .
\end{equation}
A precision measurement of the corresponding rate, relative to the
$ZZ\to 4\ell$ final state, could allow an absolute measurement of the
$b$-tagging efficiency. With a cross section $\sigma(ZZ) = 200$~pb we
expect $\sim 1.5 \cdot10^7$ ($\sim 0.5 \cdot10^7$)
$ZZ\to\ell^+\ell^-b\bar{b}$ ($ZZ\to 4\ell$) events in 20~\iab.
After including efficiencies, cuts, and even a stiff cut on $p_T(Z \to
\ell^+ \ell^-)$ to boost the recoiling $Z \to b\bar{b}$, it should be
possible to reach a sub-percent-level statistical precision.



==> 01-SM/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 01-SM/tmp.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|ccc|}
\hline 
Mode & \multicolumn{3}{c|}{Branching Fraction [$10^{-6}$]} \\
Method &  ~~NRQCD~\cite{Bodwin:2014bpa}~~ & ~~LCDA LO~\cite{Kagan:2014ila}~~
 & ~~LCDA NLO~\cite{Koenig:2015pha}~~ \\
\hline 
$\mbox{Br}(H\to\rho^0\gamma)$ & -- & $19.0\pm 1.5$ & $16.8\pm 0.8$ \\
$\mbox{Br}(H\to\omega\gamma)$ & -- & $1.60\pm 0.17$ & $1.48\pm 0.08$ \\
$\mbox{Br}(H\to\phi\gamma)$ & -- & $3.00\pm 0.13$ & $2.31\pm 0.11$ \\
$\mbox{Br}(H\to J/\psi\,\gamma)$ & $2.79\,_{-0.15}^{+0.16}$ & -- & $2.95\pm 0.17$   \\
$\mbox{Br}(H\to\Upsilon(1S)\,\gamma)$ & $(0.61\,_{-0.61}^{+1.74})\cdot 10^{-3}$ & -- 
 &  $(4.61\,_{-\,1.23}^{+\,1.76})\cdot 10^{-3}$ \\
$\mbox{Br}(H\to\Upsilon(2S)\,\gamma)$ & $(2.02\,_{-1.28}^{+1.86})\cdot 10^{-3}$  & -- 
 & $(2.34\,_{-\,1.00}^{+\,0.76})\cdot 10^{-3}$ \\
$\mbox{Br}(H\to\Upsilon(3S)\,\gamma)$ & $(2.44\,_{-1.30}^{+1.75})\cdot
10^{-3}$ & --  
 & $(2.13\,_{-\,1.13}^{+\,0.76})\cdot 10^{-3}$ \\
\hline 
\end{tabular}
\parbox{15.5cm}
{\caption{\label{table:SM_BRs} 
Theoretical predictions for the $H\to V\gamma$ branching ratios in the
SM, obtained using different theoretical approaches.}} 
\end{center}
\end{table} 



==> 02-HH/out <==
gf.tex:\includegraphics[height=.12\textwidth]{figs/ggHH_box}
gf.tex:\includegraphics[height=.12\textwidth]{figs/ggHH_tri_1}
gf.tex:\includegraphics[width=.55\textwidth]{figs/mhh_NNLL}
gf.tex:\includegraphics[width=.45\textwidth]{figs/mhh_Linear}
gf.tex:\includegraphics[width=.45\textwidth]{figs/mhh_Log}
gf.tex:\includegraphics[width=0.47\textwidth]{figs/maa_CalResolution}
gf.tex:\includegraphics[width=0.47\textwidth]{figs/mbb_CalResolution}
gf.tex:\includegraphics[width=0.47\textwidth]{figs/mbb_DelphesBfieldJES}
gf.tex:\includegraphics[width=0.493\textwidth]{figs/deltaL_vs_maa_30ab}
gf.tex:\includegraphics[width=0.495\textwidth]{figs/deltaL_vs_eta_Med_30ab}
gf.tex:\includegraphics[width=0.99\textwidth]{figs/deltaL_vs_ptag_Med_30ab}
gf.tex:\includegraphics[width=0.48\textwidth]{figs/ssb_FCC100_4b.pdf}
gf.tex:\includegraphics[width=0.48\textwidth]{figs/sb_FCC100_4b.pdf}
gf.tex:\includegraphics[width=0.43\textwidth]{figs/res_xSec_100TeV_v2}
gf.tex:\includegraphics[width=0.43\textwidth]{figs/bst_xSec_100TeV_v2}
introduction.tex:\includegraphics[width=0.55\textwidth]{figs/HH-xsec}
introduction.tex:\includegraphics[width=0.55\textwidth]{figs/HH-lam}
report.tex:% and their figures should all stay in the figs/ subdirectory
triple.tex:\includegraphics[width=0.245\textwidth]{figs/hhh_1.pdf}
triple.tex:\includegraphics[width=0.245\textwidth]{figs/hhh_2.pdf}
triple.tex:\includegraphics[width=0.245\textwidth]{figs/hhh_3.pdf}
triple.tex:\includegraphics[width=0.245\textwidth]{figs/hhh_4.pdf}
triple.tex:\includegraphics[width=0.57\textwidth]{figs/cross_hhh.pdf}
triple.tex:\includegraphics[width=0.49\textwidth]{figs/sqrts_hhh.pdf}
triple.tex:\includegraphics[width=0.49\textwidth]{figs/pt1_hhh.pdf}
triple.tex:  \includegraphics[width=0.4\textwidth]{figs/mhrec.pdf}
triple.tex:  \includegraphics[width=0.4\textwidth]{figs/mpp.pdf}
triple.tex:\includegraphics[scale=0.77]{figs/Map_nb4_M2.pdf}
triple.tex:\includegraphics[scale=0.77]{figs/Map_nb4_M5.pdf}


==> 02-HH/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}




==> 03-BSM/intro.tex <==
\subsection{Introduction}
\label{sec:DM}
In this chapter, we explore the discovery potential of BSM
Higgs sectors at a 100 TeV collider. In doing so we draw upon a rich
literature, as well as several original studies. An overview is
provided in \sref{overview}, where we briefly review some of the motivations
for BSM Higgs sectors which are explored in more detail in later sections. We also identify the most important unique physics opportunities at a 100 TeV collider, especially in connection to Higgs physics. These represent  measurements or insights into BSM scenarios that are qualitatively impossible to glean from the LHC or a lepton collider program. Finally, we argue that a 100 TeV collider is uniquely versatile as a tool for exploring BSM Higgs sectors, since it acts as both a high-energy direct production machine as well as an intensity-frontier precision tool for exploring the uncolored TeV scale. This perspective provides  guidance for future detector design, especially regarding the reconstruction of soft or exotic objects, to ensure that the full discovery potential of a 100 TeV collider is realized. 

%\DC{we originally meant to outlining the mission of a 100 TeV collider for several distinct discovery scenarios. are we still doing this?}


More detail is provided in Sections~\ref{ss.EWPT}
-~\ref{ss.naturalness}. We outline the motivation for BSM Higgs
sectors 
in the context of several unresolved mysteries: the dynamics of the
electroweak phase transition and its possible connection to
baryogenesis, the nature of dark matter, the origins of neutrino
masses, and  solutions to the Hierarchy Problem. In each case, we
identify the most promising signatures at a 100 TeV collider, and
outline the vital role such a machine would play in testing these
extensions of the SM via its exploration of BSM Higgs sectors. 

Finally, we examine the reach of a 100 TeV collider for general BSM Higgs sectors in  \ssref{bsmhiggs}, with particular attention paid to the mass reach of heavy Higgs direct production in 2HDM and singlet extensions of the SM scalar sector. Such extensions are relevant in their own right, but also occur as part of more complete theories which address the above-mentioned mysteries. The high mass reach of a 100 TeV collider makes direct  production of new Higgs states one of the most important and promising physics goals. 
%However, there are many other unique  opportunities at such a machine, and a summary is presented in~\ssref{expsummary}.  


%\DC{do we still want conclusions? points we were thinking of putting there: - 100 TeV as an Intensity Frontier Experiment: non-colored physics at 100 TeV can be sub-TeV scale, which we produce a lot of at high energies -detector and trigger requirements? [soft objects, displaced things, disappearing tracks, ..]}
%Our conclusions are summarized in~\sref{conclusions}. We argue that a 100 TeV collider is uniquely versatile as a tool for exploring BSM Higgs sectors, since it acts as both a high-energy direct production machine as well as an intensity-frontier precision tool for exploring the uncolored TeV scale. Our findings also provide guidance for future detector design, especially regarding the reconstruction of soft or exotic objects. This helps ensure the full discovery potential of a 100 TeV collider is realized. 


==> 03-BSM/nuM.tex <==
\subsection{The origin of neutrino masses\footnote{Editors: Rabi Mohapatra, Michael J. Ramsey-Musolf , Goran Senjanovich}}
\label{sec:nuM}


==> 03-BSM/report.tex <==
% Few simple rules to ensure that we you can pdfplatex your section
% locally, while maintaining the ability to pdflatex the full
% document from the home directory:

% Don't touch any of the calls in this file. 

% If you want to break the section into multiple subsection files, embed
% the \input{subsectionX} calls into the file section.tex

% Subsection files must then stay in the same folder as section.tex,
% and their figures should all stay in the figs/ subdirectory

% All references should included using the bibtex format, and must be
% added to the master report.bib file sitting in the main directory

% If you want to add new tex macros (mostly definitions or new
% commands), include them in your local section.tex file. But first
% make sure you are not overriding the macros already included in the
% main_macros.tex file sitting in the home directory. When processing
% the whole report, each subsection will then call properly its own
% macros, and properly use the master macros

% If you want to collect your macros in a file, you should then input
% it from the file section.tex or 
% from the subsection files, but it should NOT be called
% ``main_macros.tex'' (e.g. call it sectionname_macros.tex)

\input{../header}
\input{../title}
\input{../main_macros}

\input{section}

\bibliographystyle{../report}
\bibliography{../report}

\end{document}



